MotionRNN: A Flexible Model for Video Prediction with Spacetime-Varying Motions

This paper tackles video prediction from a new dimension of predicting spacetime-varying motions that are incessantly changing across both space and time. Prior methods mainly capture the temporal state transitions but overlook the complex spatiotemporal variations of the motion itself, making them difficult to adapt to ever-changing motions. We observe that physical world motions can be decomposed into transient variation and motion trend, while the latter can be regarded as the accumulation of previous motions. Thus, simultaneously capturing the transient variation and the motion trend is the key to make spacetime-varying motions more predictable. Based on these observations, we propose the MotionRNN framework, which can capture the complex variations within motions and adapt to spacetime-varying scenarios. MotionRNN has two main contributions. The first is that we design the MotionGRU unit, which can model the transient variation and motion trend in a unified way. The second is that we apply the MotionGRU to RNN-based predictive models and indicate a new flexible video prediction architecture with a Motion Highway that can significantly improve the ability to predict changeable motions and avoid motion vanishing for stacked multiple-layer predictive models. With high flexibility, this framework can adapt to a series of models for deterministic spatiotemporal prediction. Our MotionRNN can yield significant improvements on three challenging benchmarks for video prediction with spacetime-varying motions.

==> block/block_experi.tex <==
\section{Experiments}
To evaluate our proposed MotionRNN, we use three different types of datasets: the Human action dataset Human3.6M, the rader echo dataset Radar Shanghai, the synthetic dataset Moving Mnist++. These datasets contain the human, weather and synthetic varying motions. To verify the universality of MotionRNN, we use the following predictive frameworks including ConvLSTM, PredRNN, MIM and E3D-LSTM. 

The number of layers of these predictive frameworks is all set to 4. We insert three MotionRNN cells into the intervals of four layers. For E3D-LSTM, we replace the encoder and decoder inside the MotionGRU with 3D convolutions to downsample the 3D feature map to 2D and keep the other operations unchanged. In each block, the number of feature channels is set to 64. 

% For PredRNN++, we only insert two MoRNN cells into the top two intervals because the bottom interval contains the gradient high way. 

All models are trained with the $L2$ loss, using the ADAM optimizer with a learning rate of $3e^{-4}$. The momentum factor $\alpha$ is set to 0.5. The learned filter size of MotionGRU is set to $3\times$ for memory efficient. Except for E3D-LSTM, the batch size of the other models is set to 8. For E3D-LSTM, we set bacth size as 4 for Radar Shanghai and 2 for Human3.6M due to the memory limitation. Besides, we apply the scheduled sampling to all models to stitch the discrepancy between training and inference.

\subsection{Human3.6M}
The Human3.6M dataset contains the human actions of 17 different scenarios with 3.6 million poses. We follow exactly the experimental setting in MIM, including resizing the images to $128 \times 128 \times 3$, training on "walking" scenario and splitting the dataset. We use the previous 4 frames to generate the future 4 frames. 

During the human walking, the arm swinging, legs bending, body swaying, position changing and other motions could happen, which makes the prediction of real human motion a really challenging task. We present a case of human walking in Figure \ref{fig:human_exp}. In the case, each part of human body has a left movement tendency and an instantaneous change, which can be covered by our motion modeling. The frames generated with MotionRNN is richer in detail, less blurry than those of other models, especially in the arms and legs. The PredRNN and MIM present the prediction in fairly good sharpness, but fail in bending prediction of the right hand and the blur of legs. MotionRNN achieves a big progress in both sharpness and arms and legs pose prediction, which means our approach could not only maintain the details but perform well in motion capturing.

\begin{figure}[htb]
\vskip 0.15in
\centering
\includegraphics[width=\columnwidth]{cvpr2021/pic/human_exp.pdf}
\caption{Prediction examples of Human3.6M.}
\label{fig:human_exp}
\end{figure}

For quantitative results, we use the frame-wise structural similarity index measure
(SSIM), the mean square error (MSE) and the mean
absolute error (MAE) to evaluate our models. Besides, we also presents the Fr\' echet Video Distance (FVD). FVD is a metric for qualitative human judgment of generated videos and could measure both temporal coherence of the video content and the quality of each frame. Because FVD is calculated by pretrained I3D model, to match the input sequence length, we joint the input 4 frames and predicted 4 frames with repeating the first input frame twice and get a video of 9 frames finally. A lower MSE, MAE or FVD, or a higher SSIM indicates a better prediction. As shown in Table \ref{human_compare}, our proposed MotionRNN promotes the base predictive frameworks with a consistency improvement. Especially, with MotionRNN the preformance improves 29\% in MSE over PredRNN, and 22\% in MAE. Our approach also promotes the FVD, which means the prediction performs better in motion consistency and frame quality.

\begin{table}
\label{human_compare}
\begin{center}
\begin{tabular}{|l|cccc|}
\hline
Method & SSIM & MSE/10 & MAE/100 & FVD \\
\hline\hline
TrajGRU & 0.801 & 42.2 & 18.6 & 26.9 \\
Conv-TT-LSTM & 0.791 & 47.4 & 18.9 & 26.2 \\
\hline
ConvLSTM & 0.776 & 50.4 & 18.9 & 28.4 \\
\textbf{+ MotionRNN} & 0.800 & 44.3 & 18.6 & 26.9 \\
\hline
MIM & 0.790 & 42.9 & 17.8 & 21.8 \\
\textbf{+ MotionRNN} & 0.841 & 35.1 & 14.9 & 18.3 \\
\hline
PredRNN & 0.781 & 48.4 & 18.9 & 24.7 \\
\textbf{+ MotionRNN} & 0.846 & 34.2 & 14.8 & 17.6 \\
% \hline
% PredRNN++ & 0.787 & 45.3 & 18.8 & \\
% \textbf{+ MotionRNN} & 0.832 & 36.9 & 16.1 & 20.5\\
\hline
E3D-LSTM & 0.869 & 49.4 & 16.6 & 23.7 \\
\textbf{+ MotionRNN} & \textbf{0.786} & \textbf{43.8} & \textbf{18.8} & \textbf{24.7} \\
\hline
\end{tabular}
\end{center}
\caption{Quantitative results of Human3.6M.}
\end{table}

\paragraph{Memory usage analysis.}

\begin{table}
\label{human_memory_compare}
\begin{center}
\begin{tabular}{|l|cc|}
\hline
Method & Memory & GFlops \\
\hline\hline
ConvLSTM &  &   \\
\textbf{+ MotionRNN} &  &  \\
\hline
MIM & &   \\
\textbf{+ MotionRNN} &  &  \\
\hline
PredRNN &  &  \\
\textbf{+ MotionRNN} &  &  \\
\hline
E3D-LSTM &  &  \\
\textbf{+ MotionRNN} &  & \\
\hline
\end{tabular}
\end{center}
\caption{Memory usage comparison of MotionRNN.}
\end{table}

\paragraph{Ablation study.} As shown in Table \ref{human_ablation_compare}, we analyze each part of our approach. With the single Highway, we could get fairly good promotion because of the content maintaining and additional vertical spatiotemporal states transition. The only MotionGRU part gives the prediction 17\% improvement. The highway and MotionGRU make the mutual promotion. The learned motion tendency $\mathcal{D}_t^L$ gives 9\% extra promotion to the final result. This results also shows the motion consistency does matter for video prediction.


% \begin{table}
% \label{human_ablation_compare}
% \begin{center}
% \begin{tabular}{|l|cc|}
% \hline
% Method & MSE/10 & MAE/100 \\
% \hline\hline
% PredRNN & 48.4 & 18.9 \\
% \textbf{+ Highway} & 42.5 & 18.9 \\
% \textbf{+ MotionGRU} & 40.3 & 17.8 \\
% \textbf{+ MotionGRU - $\mathcal{D}_{t}^L$} & 41.5 & 18.1 \\
% \textbf{+ MotionGRU - $\mathcal{D}_{t}^L$ + Highway} & 38.9 & 16.8 \\
% \hline
% \textbf{+ MotionRNN} & 34.2 & 14.8 \\
% \hline
% \end{tabular}
% \end{center}
% \caption{The ablation of each component in MotionRNN.}
% \end{table}

\begin{table}
\label{human_ablation_compare}
\begin{center}
\begin{tabular}{|l|cc|c|}
\hline
Method & SSIM & MSE/10 & $\Delta$\\
\hline\hline
PredRNN & 0.781 & 48.4 & - \\
\textbf{+ Highway} & 0.811 & 42.5 & 12\% \\
% \textbf{+ DefConv} & 0.802 & 43.8 & 18.1 \\
% \textbf{+ SC + DefConv} & 0.824 & 38.0 & 16.6 \\
% \hline
\textbf{+ MotionGRU} & 0.805 & 40.3 & 17\% \\
\textbf{+ MotionGRU - $\mathcal{D}_{t}^L$} & 0.799 & 41.5 & 14\% \\
\textbf{+ MotionGRU - $\mathcal{D}_{t}^L$ + Highway} & 0.828 & 38.9 & 20\%\\
\hline
\textbf{+ MotionRNN} & 0.846 & 34.2 & 29\% \\
\hline
\end{tabular}
\end{center}
\caption{The ablation of each component in MotionRNN. $\Delta$ donates the MSE improvements over PredRNN.}
\end{table}

% \begin{table}
% \label{human_ablation_compare}
% \begin{center}
% \begin{tabular}{|l|ccc|}
% \hline
% Method & SSIM & MSE/10 & MAE/100 \\
% \hline\hline
% PredRNN & 0.781 & 48.4 & 18.9 \\
% \textbf{+ Highway} & 0.811 & 42.5 & 18.9 \\
% % \textbf{+ DefConv} & 0.802 & 43.8 & 18.1 \\
% % \textbf{+ SC + DefConv} & 0.824 & 38.0 & 16.6 \\
% % \hline
% \textbf{+ MotionGRU} & 0.805 & 40.3 & 17.8 \\
% \textbf{+ MotionGRU - $\mathcal{D}_{t}^L$} & 0.799 & 41.5 & 18.1 \\
% \textbf{+ MotionGRU - $\mathcal{D}_{t}^L$ + Highway} & 0.828 & 38.9 & 16.8 \\
% \hline
% \textbf{+ MotionRNN} & 0.846 & 34.2 & 14.8 \\
% \hline
% \end{tabular}
% \end{center}
% \caption{The ablation of each component in MotionRNN.}
% \end{table}



\paragraph{Learned motion visualization.}
the usage of $\mathcal{D}_t^L$. what does $\mathcal{D}_t^L$ and  $\mathcal{F}_t^L$ learned. show case of offsets, visualiization of tendency.



\subsection{Radar Shanghai}
The Radar Shanghai contains the evolving radar maps from weather bureau of Shanghai. The data were collected every 12 minutes. Each frame is a image with size $64\times 64\times 1$, covering 460 kilometers in longitude and 398 kilometers in latitude. We use the 5 frames in last 1 hour as input and predict 10 frames of the next 2 hours. For model training, we use 36000 echo sequences of 15 time steps for training and 40000 sequences as testset. As the echo data has more complex motions at each moment, such as accumulation, deformation, dissipation and diffusion and etc., the prediction needs more motion information.

As presented in Figure \ref{fig:radar_exp}, MotionRNN generates the predictions with more accuracy. In the top case, there is a cyclone with the motion contains moving up and anticlockwise rotation. PredRNN could roughly predict the cyclone positions, but suffers the bur. Focusing on the center part of prediction at $t=15$, MotionRNN forecasts the exact rotation trend, but the echoes predicted from PredRNN is just a block without cyclone rotation details. In the bottom case, the echoes have a up diffusion movement and a slight anticlockwise rotation simultaneously. Our approach provides more details for the diffusion than PredRNN. We can find many small cloud clusters in the right-bottom area and more subtle outline of the center part.

\begin{figure}[htb]
\vskip 0.15in
\centering
\includegraphics[width=\columnwidth]{cvpr2021/pic/radar_exp.pdf}
\caption{Examples of the future two hours predictions of radar echoes. For better vision, we did the colour modulation to the frames, where the higher R value in these RGB frames indicate higher precipitation probabilities.}
\label{fig:radar_exp}
\end{figure}

Besides the regular pixel-wise metric MSE, we use the gradient difference loss (GDL) to measure the sharpness of our predictions. A lower GDL indicates a higher sharpness similarity of ground truth. For radar echo intensities, we convert the pixel values in dBZ and compare the Critical Success Index (CSI) with 30 dBZ, 40 dBZ, 50 dBZ as thresholds respectively. CSI is defined as $\frac{\text{Hits}}{\text{Hits}+\text{Misses}+\text{FalseAlarms}}$, where hits correspond to the true positive, misses correspond to the false positive, and false alarms correspond to the false
negative. A higher CSI indicates the better forcasting. The quantitative results are shown in Table \ref{rader_compare}. With MotionRNN, the predictive frameworks get a significant improvement. For the state-of-the-art model E3D-LSTM, our approach achieves 46\% improvement in MSE.

\begin{table}
\label{rader_compare}
\begin{center}
\begin{tabular}{|l|ccccc|}
\hline
Method & MSE & GDL & CSI30 & CSI40 & CSI50 \\
\hline\hline
TrajGRU & 8.01 & 13.9 & 0.576 & 0.545 & 0.484  \\
Conv-TT-LSTM & 8.35 & 13.6 & 0.571 & 0.530 & 0.469 \\
\hline
ConvLSTM & 6.55 & 12.6 & 0.624 & 0.605 & 0.560 \\
\textbf{+ MotionRNN} & 5.84 & 11.9 & 0.646 & 0.629 & 0.586 \\
\hline
MIM & 5.66 & 11.3  & 0.654 & 0.646 & 0.609 \\
\textbf{+ MotionRNN} &  &  &  &  &  \\
\hline
PredRNN & 6.34 & 11.9 & 0.633 & 0.622 & 0.581 \\
\textbf{+ MotionRNN} & 4.91 & 10.9 & 0.678 & 0.664 & 0.623 \\
% \hline
% PredRNN++ & 5.81 & & 0.647 & 0.629 & 0.589 \\
% \textbf{+ MotionRNN} & 4.96 & 10.8 & 0.678 & 0.668 & 0.633 \\
\hline
E3D-LSTM & 7.48 & 12.7 & 0.615 & 0.615 & 0.590\\
\textbf{+ MotionRNN} & 4.02 & 9.67 & 0.671 & 0.659 & 0.621 \\
\hline
\end{tabular}
\end{center}
\caption{radar Results.}
\end{table}

\paragraph{Learned motion visualization.} For have a better view of learned motion tendency, we visualized the $\mathcal{D}_{t}^1$, the hidden state of the first layer MotionGRU. As the input is with size $64\times 64\times 1$, after the patch operation with 4 patch number and the encoder with stride 2 inside the MotionGRU, $\mathcal{D}_{t}^1$ is with size $8\times 8\times 18$, where the kernel size is 3. And $\mathcal{D}_{t}^1$ can be separated into two tensors, each of them has the size of $8\times 8\times 9$ and presents the learned offsets of $3\times 3$ filter in x-axis and y-axis respectively. First, we calculate the mean along the channel dimension and get two $8\times 8$ variances for the x-offset and y-offset of every pixel of the $8\times 8$ feature map. After the length regularization, we use the arrows to show the opposite direction of the offsets, which is just the motion tendency. The visualization is shown in Figure \ref{fig:radar_show}. For simplify, we just show the offsets with above average values without any other selection conditions. At $t=1$, the direction of arrows is with great randomness, but with the time moving, the direction reflect the motion of echoes exactly. At $t=15$, the bottom arrow shows the down motion of the little tile of cyclone, which is match the human expectation. And the arrows of right parts point to up-right, which matchs the diffusion direction of the cyclone. This visualization exactly shows that MotionRNN could capture the sustainable motion tendency and that is the explanation of our approach could adapt to the varying motion in echoes.

\begin{figure}[htb]
\vskip 0.15in
\centering
\includegraphics[width=\columnwidth]{cvpr2021/pic/radar_show.pdf}
\caption{The visualization of learned motion tendency. The arrows are calculated from the model hidden variance  $\mathcal{D}_t^L$ and show the opposite direction of kernel offests.}
\label{fig:radar_show}
\end{figure}

\subsection{Moving MNIST++}
The original Moving MNIST dataset just contains the digits moving with a constant speed and is not suitable for evaluating varying motions. Thus we generate the Moving MNIST++ dataset following the operations in TrajGRU. The dataset in TrajGRU is in low speed and the occlusion rarely occurs. We generated the new Moving MNIST++ dataset with  2 moving digits, moving speed in range [1.0, 3.6], scaling in range [0.95, 1.05] and rotations. We generate $1e^5$ sequences with $64\times 64\time 1$ frame size of and 20 time steps for training and $1e^4$ sequences as the testset. 




\begin{table}
\label{human_compare}
\begin{center}
\begin{tabular}{|l|cccc|}
\hline
Method & MSE & SSIM & PSNR & GDL \\
\hline\hline
TrajGRU & 109 & 0.515 & 15.9 & 69.3 \\
Conv-TT-LSTM &  &  &  &   \\
\hline
E3D-LSTM & 57.6 & 0.852 & 19.72 & 44.6 \\
\textbf{+ MotionRNN} & & & & \\

\hline
ConvLSTM & 47.0 & 0.845 & 20.6 & 41.8 \\
\textbf{+ MotionRNN} & 44.4 & 0.861 & 20.9 & 40.3 \\

\hline
MIM & 34.6 & 0.888 & 22.3 & 34.6 \\
\textbf{+ MotionRNN} &  &  &  &   \\

\hline
PredRNN & 35.6 & 0.891 & 22.1 & 34.7  \\
\textbf{+ MotionRNN} & 25.1 & 0.920 & 24.0 & 27.7  \\
% \hline
% PredRNN++ & & & &  \\
% \textbf{+ MotionRNN} & & & & \\

\hline
\end{tabular}
\end{center}
\caption{Moving Mnist++ Results.}
\end{table}


==> block/block_method.tex <==
\section{Methods}
%Real-world motions are complicated and erratic, which can be regarded as the entanglement of series transitions, such as translation, rotation, deformation, etc. 


%In this section, we provide a solution to capture the entanglement of current transformation and video tendency. Different from most previous video prediction methods,

%In this section, we provide a novel spatiotemporal operator \textit{MotionRNN}, which can give consideration to both current transformation and video tendency. The MotionRNN could adapt to diverse predictive frameworks and varying video motions.


%It could enhance the state transition of normal LSTM-stacked-based predictive frameworks with explicit receptive filed changing. With high flexibility, our approach can adapt to diverse predictive frameworks and varying video motions.


%In this section, we provide detailed descriptions of the \textit{MotionRNN} framework.
% As described in Figure \ref{fig:human_show}, we can see that varying motions are the decomposition of \textit{instantaneous motion variations} and the \textit{sustainable motion tendency}. We believe that a spatiotemporal predictive system should capture instantaneous variations and maintain the motion's sustainable tendency. In this section, we provide the descriptions of a novel \textit{MotionRNN} framework, a new recurrent unit named \textit{MotionGRU} and the \textit{Motion Content Highway (MCH)}. 

%for compensating the necessary content. 

%\subsection{MotionRNN Framework}

%which adapts the MotionGRU unit to existing predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn}. The MotionGRU could generate the instantaneous filter for the rapidly changing varying motion and make the sustainable motion tendency can be incorporate into the unit using the sustainable momentum learner. In addition, our MotionRNN also applys the \textit{Motion Content Highway} to enhancing the state transition across layers for maintaining the background information of the varying motion. Our approach with high flexibility can adapt to diverse predictive frameworks and varying video motions. 

%In this section, we first introduce the \textit{MotionGRU} unit, which could generate the instantaneous filter for the rapidly changing varying motion and make the sustainable motion tendency can be incorporate into the unit using the sustainable momentum learner. Then we discuss a new framework \textit{MotionRNN}, which adapts the MotionGRU unit to existing predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn}. The MotionRNN also applys the \textit{Motion Background Highway} to enhancing the state transition across layers for maintaining the background information of the varying motion. Our approach with high flexibility can adapt to diverse predictive frameworks and varying video motions. 

% As described in Figure \ref{fig:human_show}, we can see that varying motions are the decomposition of \textit{instantaneous motion variations} and the \textit{sustainable motion tendency}. We believe that a spatiotemporal predictive system should capture instantaneous variations and maintain the motion's sustainable tendency. In this section, we provide the descriptions of a novel \textit{MotionRNN} framework, a new recurrent unit named \textit{MotionGRU} and the \textit{Motion Content Highway (MCH)}. 

As shown in Figure \ref{fig:human_show}, real-world motions can be decomposed to transient variations and the motion trend. Enlightened by this observation, we propose the flexible framework MotionRNN with a motion highway, which could effectively enhance the ability to adapt to the spacetime-varying motions and avoid the motion vanishing. Furthermore, we propose a specifically designed unit MotionGRU, which can capture the transient variation and motion trend in a unified cell. This section will first describe the proposed MotionRNN architecture and illustrate how to adapt MotionRNN to the existing RNN-based predictive models. Next, we will show the transient variation and motion trend modeling in the MotionGRU unit.

% As described in Figure \ref{fig:human_show}, we can see that varying motions are the decomposition of \textit{instantaneous motion variations} and the \textit{sustainable motion tendency}. We believe that a spatiotemporal predictive system should capture instantaneous variations and maintain the motion's sustainable tendency. In this section, we provide the descriptions of a novel \textit{MotionRNN} framework, a new recurrent unit named \textit{MotionGRU} and the \textit{Motion Content Highway (MCH)}. 

\subsection{MotionRNN}
The RNN-based spatiotemporal predictive frameworks are always in the form of stacked blocks, as shown in Figure \ref{fig:pipeline}. In this framework, the hidden states transit between predictive blocks and controlled by the inner gates. However, when it comes to spacetime-varying motions, the gate-controlled information flow would fail in quick response for transient variation, as the statements in MIM \cite{WangZZLWY19} that the forget gates are easily saturated. Besides, it also lacks motion trend modeling.

\begin{figure}[htb]
\centering
\includegraphics[width=1\columnwidth]{cvpr2021/pic/pipeline-final-new.pdf}
\caption{
An overview of the architecture of predictive frameworks: RNN-based spatiotemporal predictive networks (\textbf{left}), MotionRNN framework (\textbf{right}) which embeds the MotionGRU (\textcolor{blue}{blue} circles) between layers. The \textcolor{blue}{blue} dashed lines between stacked layers present the motion highway.
%MotionGRU is used as an operator to the vertical spatiotemporal flow. The blue dashed lines between stacked layers presents the motion content highway.
}
\label{fig:pipeline}
\end{figure}

To tackle the challenge of spacetime-varying motions modeling, the MotionRNN framework incorporates the MotionGRU unit between the stacked layers as an operator without changing the original state transition flow (Figure \ref{fig:pipeline}). MotionGRU can capture the motion and conduct a state transition to the hidden states based on the learned motion. However, we find that motion will blur even vanish when the transited feature passes through multi-layers. Motivated by this observation, MotionRNN introduces the motion highway to provide an alternative quick route for the motion content information. We can find that motion highway could avoid motion blur and constrain the object in the right area effectively from the visualization in Figure \ref{fig:human_mc}.


For details, the MotionRNN framework inserts the MotionGRU between layers. Take the ConvLSTM \cite{shi2015convolutional} as an example. After the first block layer, the overall equations for the $l$-th layer at $t$ time step are as follows:
\begin{equation}\label{equ:overall}
  \begin{split}
    & \mathcal{X}_{t}^{l-1}, \mathcal{F}_{t}^{l-1}, \mathcal{D}_{t}^{l-1} = \textrm{MotionGRU}(\mathcal{H}_{t}^{l-1}, \mathcal{F}_{t-1}^{l-1}, \mathcal{D}_{t-1}^{l-1}) \\
    & \mathcal{H}_{t}^{l}, \mathcal{C}_{t}^{l} = \textrm{Block}(\mathcal{X}_{t}^{l-1}, \mathcal{H}_{t-1}^{l}, \mathcal{C}_{t-1}^{l}) \\
    & \mathcal{H}_{t}^{l} = \mathcal{H}_{t}^{l}+(1-o_{t})\odot\mathcal{H}_{t}^{l-1}, \\
  \end{split}
\end{equation}
where $l\in \{2, 3,\cdots, L\}$. $\mathcal{F}_{t}^{l-1}$ and $\mathcal{D}_{t}^{l-1}$ donate the learned motion filter and the trending momentum from MotionGRU respectively. MotionGRU explicitly transits $\mathcal{H}_{t}^{l-1}$ to $\mathcal{X}_{t}^l$ based on the learned motion information. We will give detailed descriptions to MotionGRU in the next section. The input $\mathcal{X}_{t}^{l-1}$ of the Block has been transited by MotionGRU. $\mathcal{H}_{t-1}^{l}$, $\mathcal{C}_{t-1}^{l}$ are the hidden state and memory state from the previous time step, which is the same as original predictive blocks. $o_t$ donates the output gate of the RNN-based predictive block. 

The last equation presents the motion highway, which compensates the predictive block's output with the previous hidden state $\mathcal{H}_{t}^{l-1}$ by reusing the output gate. This highway connection provides extra details to the hidden states and balance the invariant part and the changeable motion part.

Note that our MotionRNN does not change the original state transition flow in the predictive models. Thus, with high flexibility, MotionRNN can adapt to diverse predictive frameworks such as ConvLSTM \cite{shi2015convolutional}, PredRNN \cite{wang2017predrnn}, MIM \cite{WangZZLWY19}, E3D-LSTM \cite{wang2019eidetic}, and other RNN-based predictive models. It can significantly enhance spacetime-varying motion modeling based on existing predictive models.

% With the original predictive block unchanged, we adapt the MotionGRU and MCH into the framework.

%\subsection{MotionRNN Framework}
%\begin{figure}[htb]
%\vskip 0.15in
%\centering
%\includegraphics[width=\columnwidth]{cvpr2021/pic/pipeline-final-new.pdf}
%\caption{Predictive Framework with 3 layers: RNN-based networks (left), MotionRNN framework (center) which embeds MotionGRU into networks and a close look of connections of MotionGRU between layers. Our approach incorporates the MotionGRU (blue circles) into regular predictive models without change the spatiotemporal flow. MotionGRU is used as an operator to the vertical spatiotemporal flow. The blue dashed lines between stacked layers presents the Motion Content Highway.}
%\label{fig:pipeline}
%\end{figure}


%for maintaining the overall video tendency at the same time. We then discuss a new RNN architecture, which adapts the MotionRNN unit to existing predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn}. Our approach with high flexibility can adapt to diverse predictive frameworks and varying video motions.



%enhancing the state transition with explicit receptive field changes and 

%maintaining the overall video tendency at the same time. We then discuss a new RNN architecture, which adapts the MotionRNN unit to existing predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn}. Our approach with high flexibility can adapt to diverse predictive frameworks and varying video motions.



%the entanglement of series transitions (etc. \textit{translation}, \textit{rotation} and \textit{deformation}), our MotionRNN considers both current transformation and video tendency.
%Thus, we adapt the MotionRNN unit to existing predictive networks such as ConvLSTM and PredRNN, enhancing the state transition with explicit receptive field changes.

%Compared with other predictive networks, our approach performs better in above varying motion situation with two key insights: First, it presents a new spatial temporal operator MoRNN unit which can give consideration to both current transformation and video tendency. Second, it enhances the state transition of normal LSTM-stacked-based predictive frameworks with explicit receptive filed changing. With high flexibility, our approach can adapt to diverse predictive frameworks and varying video motions.


\subsection{MotionGRU}

As mentioned above, towards modeling the spacetime-varying motions, our approach presents the MotionGRU unit to conduct motion-based state transitions by modeling the transient variation and trend of the motion.
In video prediction, the motion can be presented as pixels displacement corresponding to the hidden states transitions in RNNs. Here we use the MotionGRU to learn the pixel offsets between adjacent states. The learned pixel-wise offsets are donated by motion filter $\mathcal{F}_{t}^l$. Considering that real-world motions are the composition of transient variations and motion trends, we specifically design two modules in the MotionGRU to model these two 
components respectively (Figure \ref{equ:mornn_unit}). 

% Predicting varying motions is a challenging task for video prediction. Based on the insight of motion decomposition mentioned before, the spatiotemporal predictive model needs to consider the sustainable motion tendency of the whole video and the instantaneous variation of the motion simultaneously. Motivated by these concerns, our approach presents the MotionGRU unit, which contains a learned filter with instantaneous spatiotemporal variation information and a constantly optimized sustainable motion tendency. As shown in Figure \ref{fig:mornn_unit}, the main architecture of \textit{MotionGRU} has two components: an \textit{instantaneous filter learner} and a \textit{sustainable momentum updater}. For memory efficiency, our MotionGRU employs an Encoder-Decoder structure.

%Previous spatiotemporal predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn} mainly focus on capturing the overall motion tendency of the video.  These methods only use the convolution kernel for the spatial temporal transition. The fixed quadrate receptive fields of normal CNNs could not capture the deformable instantaneous variation. For example, when it comes to fast movement, deformation and other varying motions, these predictive models may behave worse. TrajGRU \cite{shi2017deep} and non-local ConvLSTM \cite{xu2019non} take the whole feature map into account, but overlook the origin motion consistency in videos which could make the transition with more randomness. 

%Considering this property of video motions, our approach presents the MotionRNN unit which contains a learned filter with temporal information.



%from the long-term view, we find the subject motions follow a tendency with high consistency but random offsets in short-term.

%Previous predictive networks such as ConvLSTM, PredRNN only use the convolution kernel for the spatial temporal transition. The fixed quadrate receptive fields of normal CNNs restrict the video motion modeling. Thus when it comes to fast movement, deformation and other varying motions, these networks could fail. TrajGRU and other non-local networks take the whole feature map into account, but neglected the origin motion consistency in videos which could make the transition with more randomness. Considering this property of video motions, our approach presents the MoRNN unit which contains a learned filter with temporal information.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\columnwidth]{cvpr2021/pic/block-new-final-warp.pdf}
\caption{MotionGRU unit's architecture. The \textcolor{blue}{blue} part is to capture the transient variation $\mathcal{F}_{t}^\prime$.
The trending momentum $\mathcal{D}_{t}^L$ accumulates the motion tendency in a momentum way (\textcolor{red}{red} part).}
\vspace{-10pt}
\label{fig:mornn_unit}
\end{figure}

% \vspace{-10pt}
\subsubsection{Transient Variation} 

% The idea of capturing deformable transitions is initially inspired by the deformbale convolution networks \cite{dai2017deformable}. The deformable convolution network adds 2D spatial offset to the regular grid sampling locations for free form deformation, but could not capture the temporal variations from the motion. Different from the deformable convolutional networks, 

In a video, the transient variation at each time step is not only based on the spatial context but also presents high temporal coherence. For example, the waving hands of a man follow a nearly continuous arm rotation angle between adjacent frames. Motivated by the spatiotemporal coherence of motion variations, we adapt a ConvGRU \cite{shi2017deep} to learn the transient variation. With this convolutional recurrent network, the learned transient variation could consider the instant states and maintain the spatiotemporal coherence of variations. The equations of the transient-variation learner of $l$-th MotionGRU at $t$ time step are shown as follows:
% The transient filter learner is specifically designed to produce the filter for instantaneous motion variations, \textit{e.g.} speed reduction, direction-changing. It uses the ConvGRU \cite{shi2017deep} to learn the spatiotemporal variation, which can incorporate the temporal information and spatial content simultaneously. Thus it can maintain the spatiotemporal coherence of variations. The equations of the instantaneous filter learner are shown as follows:
\begin{equation}\label{equ:motionGRU_unit}
  \begin{split}
  & u_t = \sigma\Big(W_{u}\ast \text{Concat}([\text{Enc}(\mathcal{H}_t^l), \mathcal{F}_{t-1}^l])\Big) \\
  & r_t = \sigma\Big(W_{r}\ast \text{Concat}([\text{Enc}(\mathcal{H}_t^l), \mathcal{F}_{t-1}^l])\Big) \\
  &z_t = \tanh\Big(W_{z}\ast \text{Concat}([\text{Enc}(\mathcal{H}_t^l), r_t \odot \mathcal{F}_{t-1}^l])\Big) \\
  & \mathcal{F}_t^\prime =  u_t \odot z_t 
   + (1-u_t) \odot \mathcal{F}_{t-1}^l, \\
  \end{split}
\end{equation}
where $\sigma$ is the sigmoid function, $W_{u}$, $W_{r}$ and $W_{z}$ donates the $1\times 1$ convolution kernel, $\ast$ and $\odot$ denote the convolution and the Hadamard product respectively. $\text{Enc}(\mathcal{H}_{t}^l)$ donates the input from the last predictive block and through the encoder. $\mathcal{F}_{t-1}^l$ presents motion filter from the previous time step. $u_t$ and $r_t$ donate the update gate and reset gate. $z_t$ presents the rested feature of current moment. Transient variation $\mathcal{F}_{t}^\prime$ for current frame is from $\mathcal{F}_{t-1}^l$ and $z_t$ and controlled by the update gate $u_t$. Note that transient variation $\mathcal{F}_{t}^l$ presents the transition of each pixel's position between adjacent states. Thus, except for the input $\text{Enc}(\mathcal{H}_{t}^l)$, all the gates, $z_{t}$, and $\mathcal{F}_{t}^l$ are in the offset space. 


% where all these gates and hidden states belong to $\mathbb{R}^{2k^2\times \frac{H}{2}\times \frac{W}{2}}$. Note that the output $\mathcal{F}_{t}^\prime$ is instantaneous but still keep the spatiotemporal coherence of previous motion filters by the recurrent structure.


\subsubsection{Trending Momentum} 

In the running scenario, the man's body sways up and down at each step while the man keeps moving forward. In this case, the motion is following a forward trend. In video prediction, we usually have to go through the whole frame sequence to get the motion trend. However, the future is unreachable. This dilemma is similar to reward prediction in reinforcement learning. Enlightened by \textit{Temporal Difference} \cite{sutton1988learning}, we use an accumulating way to get the pattern of motion variation. We use the previous motion filter $\mathcal{F}_{t-1}^l$ as the estimation of the current motion trend and get the momentum update function as follows:
\begin{equation}\label{equ:dynamic}
  \begin{split}
  & \mathcal{D}_{t}^l = \mathcal{D}_{t-1}^l + \alpha (\mathcal{F}_{t-1}^l - \mathcal{D}_{t-1}^l), \\
  \end{split}
\end{equation}
where the $\alpha$ is the step size of momentum update, $\mathcal{D}_{t}^l$ donate the learned trending momentum. With momentum update, $\mathcal{D}_{t}^l$ convergences to the weighted sum of motion filter $\mathcal{F}_{t}^l$, which can be viewed as the motion trend in the past period. In the running case, $\mathcal{F}_{t-1}^l$ presents the motion of the last moment and $\mathcal{D}_{t}^l$ donates the forward trend learned from the past. By momentum updating, this tendency estimation is with more coefficient across time. In addition, the accumulation process can also reduce the variance of the learned motion filter significantly and perform as a stabilizer for spacetime-varying motion modeling. Note that the trending momentum $\mathcal{D}_{t}^l$ is the momentum update of motion filter $\mathcal{F}_{t}^l$ and is also in the offset space. $\mathcal{D}_{t}^l$ presents the learned motion trend of pixels in a video.



\subsubsection{Overall Procedure for MotionGRU} 

Based on the motion decomposition shown in Figure \ref{fig:human_show}, we build the MotionGRU as follows:
\begin{equation}\label{equ:mornn_unit}
  \begin{split}
  & \mathcal{F}_{t}^\prime = \textrm{Transient}\Big(\mathcal{F}_{t-1}^l, \textrm{Enc}(\mathcal{H}_{t}^l)\Big)\\
  & \mathcal{D}_{t}^l = \textrm{Trend}\Big(\mathcal{F}_{t-1}^l, \mathcal{D}_{t-1}^l\Big)\\
  & \mathcal{F}_{t}^l = \mathcal{F}_{t}^\prime + \mathcal{D}_{t}^l \\
  & m_{l} = \textrm{Broadcast}\Big(\sigma(W_\textrm{hm}\ast \textrm{Enc}(\mathcal{H}_{t}^l))\Big) \\
  & \mathcal{H}_t^\prime = m_t \odot \textrm{Warp}\Big(\textrm{Enc}(\mathcal{H}_{t}^l), \mathcal{F}_{t}^l\Big)\\
  & g_{t} = \sigma \Big(W_{hg}\ast \textrm{Concat}([\textrm{Dec}(\mathcal{H}_t^\prime ), \mathcal{H}_{t}^{l}])\Big) \\
  & \mathcal{X}_{t}^l = g_{t}\odot \mathcal{H}_{t-1}^l + (1-g_{t})\odot \textrm{Dec}(\mathcal{H}_t^\prime),\\
  \end{split}
\end{equation}
where the subscript $t$ denotes the time step and the superscript $l\in\{2, \cdots, L\}$ denotes the current layer number, $W_{hg}$ and $W_{hm}$ donate the convolution kernel. \textrm{Transient} and \textrm{Trend} present the transient-variation learner and trending-momentum updater respectively. $\mathcal{F}_{t}^\prime$ and $\mathcal{D}_{t}^l$ donates the transient variation and trending momentum of current frame. The motion filter $\mathcal{F}_{t}^l$ is the combination of transient variation and trending momentum. $m_t$ is the mask for motion filter and we use the broadcast operation to keep tensor dimension consistent to $\mathcal{H}_{t}^\prime$.
\begin{figure}[htb]
\centering
\includegraphics[width=\columnwidth]{cvpr2021/pic/unit.pdf}
\caption{State transitions by MotionGRU. The motion filter $F_{t}^l$ is the combination of the transient variation (\textcolor{blue}{blue} square) and trending momentum (\textcolor{red}{red} square). The transited state $\mathcal{X}_{t}^l$ is obtained by the warp operation based on the learner motion filter.}
\label{fig:offset_show}
\end{figure}

For the state transition, we use the warp operation \cite{black1996robust, brox2004high} to map the pixels from previous state to the position in the next state, which is widely used in different fields of video analysis, such as video style transfer \cite{chen2017coherent} and video restoration \cite{wang2019edvr}. Here \textrm{warp} donates the warp operation with bilinear interpolation. 
% It can select the pixels in $\text{Enc}(\mathcal{H}_{t}^l)$ by the learned motion filter $F_{t}^l$, which also presents the motion of pixels.
As shown in Figure \ref{fig:offset_show}, warping the previous state by the learned motion $\mathcal{F}_{t}^l$, we can explicitly incorporate motion variation into the transition of hidden states. More details about the warp operation in MotionGRU can be found in the supplementary material.
%
At last, the final output $\mathcal{X}_{t}^l$ of MotionGRU is a gate-controlled result from the input $\mathcal{H}_{t}^l$ and the decoder output, in which the decoder output has been already explicitly transited by warp operation based on the motion $\mathcal{F}_{t}^l$.

All in all, by capturing and fusing the transient variation and motion trend separately, MotionGRU can effectively model the spacetime-varying motions. With MotionGRU and motion highway, our proposed MotionRNN framework can be applied to the scenarios with changeable motions.

% Unlike previous RNN-based blocks updating the memory cell to capture dynamics, our MotionGRU could dynamically generate the instantaneous filter $\mathcal{F}_{t}^\prime$ to incorporate instantaneous spatial and temporal variations.  



% The \textrm{Broadcast} means the operation to broadcast and transpose the $k^2\times H^\prime\times W^\prime$ tensor to $C^\prime\times H^\prime\times W^\prime\times k^2$. $m_t$ is the mask for the motion of the $k \times k$ filter area. 
% The \textrm{Warp} donates the warp operation with bilinear interpolation. It can select the pixels in $\text{Enc}(\mathcal{H}_{t}^L)$, which point out to the $k\times k$ filter area by offset $F_{t}^L$. The warp operation is widely used in different fields of video analysis, such as video style transfer \cite{chen2017coherent} and video restoration \cite{wang2019edvr} , which can be formulated as follows:
% \begin{equation}\label{equ:mornn_unit_warp}
%   \begin{split}
%   & \text{Warp}(\mathcal{H}, \mathcal{F}) = \Big(\mathcal{H}_{c,m,n,i}^\prime\Big)_{C^\prime\times H^\prime\times M^\prime\times k^2}  \\  & = \Big(\mathcal{H}_{c,(m+p_{ix}-\mathcal{F}_{i,m,n}),(n+p_{iy}-\mathcal{F}_{i+k^2,m,n})}\Big)_{C^\prime\times H^\prime\times M^\prime\times k^2}, \\
%   \end{split}
% \end{equation}
% where $i\in\{1,2,\cdots,k^2\}$, $p_{ix}=[\frac{i}{k}]-[\frac{k}{2}]$, $p_{iy}=(i\ \text{mod}\ k)-[\frac{k}{2}]$. The decoder squeezes $\mathcal{H}_{t}^\prime$ to encoded feature field by $1\times 1$ convolution and deconvolution to feature field. More details about the warp operation can be found in supplementary material.











% \subsection{Motion Content Highway}
% Because of the encoder-decoder structure in MotionGRU, the incorporation of MotionGRU causes the information bottleneck for frame details. We upgrade the predictive framework by adding the MCH after stacked blocks, which provides an alternative quick route for the content information of the varying motion. 
% Besides, this highway could refine the motion and avoid motion vanishing. 
% Take ConvLSTM as an example, the original inputs are $\mathcal{X}_{t}^{L-1}$ from frames or previous block, hidden state $\mathcal{H}_{t-1}^L$ and memory state $\mathcal{C}_{t-1}^{L}$ from previous time step, 
%and the original outputs are $\mathcal{H}_{t}^L$, $\mathcal{C}_{t}^L$, 
% Take ConvLSTM as an example, the original inputs are $\mathcal{X}_{t}^{L-1}$ from frames or previous block, hidden state $\mathcal{H}_{t-1}^L$ and memory state $\mathcal{C}_{t-1}^{L}$ from previous time step, 
% where the subscript $t$ denotes the time step and the superscript $L\in\{1,2, \cdots, K\}$ denotes the $L$-th hidden layer in a stacked predictive framework. In MotionRNN, the input $\mathcal{X}_{t}^{L-1}$ is from the frames or previous MotionGRU and with the additional \textit{Motion Content} $\mathcal{H}_{t}^{L-1}$. MCH uses $\mathcal{H}_t^{L-1}$ to compensate the output of the original block as follows:
% We take the ConvLSTM as an example. The original outputs are hidden states $\mathcal{H}_{t}^L$ and memory states $\mathcal{C}_{t}^{L}$, where the subscript $t$ denotes the time step and the superscript $L\in\{1,2, \cdots, K\}$ denotes the $L$-th hidden layer in a stacked predictive framework. In MotionRNN, the output hidden states $\mathcal{H}_{t}^{L}$ from previous ConvLSTM are compensated by the additional \textit{Motion Content} $\mathcal{H}_{t}^{L-1}$. MCH uses $\mathcal{H}_t^{L-1}$ to refine the output of the original block as follows:
% \begin{equation}\label{equ:block_new}
%   \begin{split}
%     & \mathcal{H}_t^L = \mathcal{H}_{t}^L + (1-o_t) \odot \mathcal{H}_t^{L-1},\\
%   \end{split}
% \end{equation}
% where we reuse the output gate $o_t$ in RNNs to control the spatiotemporal flow for the balance of motion and content information.

% As shown in Figure \ref{fig:offset_show}, the MotionRNN learns the spatiotemporal variation with instantaneous filter and sustainable momentum, which could capture both the instantaneous transformation and motion tendency. Our MotionRNN performs better in varying motions by learning instantaneous and sustainable variations explicitly. 




% \begin{figure*}[h]
% \vskip 0.05in
% \centering
% \subfigure[Incorporate into Prediction Nets]{
% \includegraphics[width=0.8\columnwidth]{cvpr2021/pic/pipeline.pdf}
% \label{fig:stacked_convlstm}
% }
% \hspace{2cm}
% \subfigure[MoRNN Block]{
% \includegraphics[width=0.65\columnwidth]{cvpr2021/pic/block.pdf}
% \label{fig:deeplstm}
% }
% \caption{
% The diagram is a case of 3 layers network. Normal predictive deep networks can be view as stacked LSTM blocks, which is the black part in (a). The blue part in (a) shows the approach to incorporating MoRNN into these networks by using it as a flexible operator to $\mathcal{H}_{t}^L$ and adding vertical spatial temporal skip connection as a stabilizer. MoRNN (b) models the motions with \textcolor{blue}{GRU block} and \textcolor{red}{
% Momentum block} to capture the deformation and tendency respectively}
% \label{fig:model_comparison}
% \end{figure*}




==> block/block_method_1.tex <==
\section{MotionRNN}
%Real-world motions are complicated and erratic, which can be regarded as the entanglement of series transitions, such as translation, rotation, deformation, etc. 


%In this section, we provide a solution to capture the entanglement of current transformation and video tendency. Different from most previous video prediction methods,

%In this section, we provide a novel spatiotemporal operator \textit{MotionRNN}, which can give consideration to both current transformation and video tendency. The MotionRNN could adapt to diverse predictive frameworks and varying video motions.


%It could enhance the state transition of normal LSTM-stacked-based predictive frameworks with explicit receptive filed changing. With high flexibility, our approach can adapt to diverse predictive frameworks and varying video motions.


%In this section, we provide detailed descriptions of the \textit{MotionRNN} framework.
As shown in Figure \ref{fig:human_show}, we can see that varying motions are the decomposition of \textit{instantaneous motion variations} and the \textit{sustainable motion tendenncy}. We believe that a spatiotemporal predictive system should capture varying instantaneous variations and maintain the sustainable tendency of the motion in a unified unit. In this section, we first introduce the \textit{MotionGRU} unit, which could generate the instantaneous filter for the rapidly changing varying motion and make the sustainable motion tendency can be incorporate into the unit using the sustainable momentum learner. Then we discuss a new framework \textit{MotionRNN}, which adapts the MotionGRU unit to existing predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn}. The MotionRNN also applys the \textit{Motion Background Highway} to enhancing the state transition across layers for maintaining the background information of the varying motion. Our approach with high flexibility can adapt to diverse predictive frameworks and varying video motions. 


%for maintaining the overall video tendency at the same time. We then discuss a new RNN architecture, which adapts the MotionRNN unit to existing predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn}. Our approach with high flexibility can adapt to diverse predictive frameworks and varying video motions.



%enhancing the state transition with explicit receptive field changes and 

%maintaining the overall video tendency at the same time. We then discuss a new RNN architecture, which adapts the MotionRNN unit to existing predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn}. Our approach with high flexibility can adapt to diverse predictive frameworks and varying video motions.



%the entanglement of series transitions (etc. \textit{translation}, \textit{rotation} and \textit{deformation}), our MotionRNN considers both current transformation and video tendency.
%Thus, we adapt the MotionRNN unit to existing predictive networks such as ConvLSTM and PredRNN, enhancing the state transition with explicit receptive field changes.

%Compared with other predictive networks, our approach performs better in above varying motion situation with two key insights: First, it presents a new spatial temporal operator MoRNN unit which can give consideration to both current transformation and video tendency. Second, it enhances the state transition of normal LSTM-stacked-based predictive frameworks with explicit receptive filed changing. With high flexibility, our approach can adapt to diverse predictive frameworks and varying video motions.


\subsection{MotionGRU}
For predicting the varying motion of the video more precisely, the spatiotemporal predictive model not only needs to concentrate on the sustainable motion tendency of the whole video but also has to care about the instantaneous trend of the motion. Motivated by these concerns, our approach presents the MotionGRU unit which contains a learned filter with instantaneous spatiotemporal variation information and always remembers the sustainable motion tendency. As shown in Figure \ref{equ:mornn_unit}, the main architecture of \textit{MotionGRU} has two components: an \textit{instantaneous filter learner} and a \textit{sustainable momentum learner}. 

%Previous spatiotemporal predictive networks such as ConvLSTM \cite{shi2015convolutional} and PredRNN \cite{wang2017predrnn} mainly focus on capturing the overall motion tendency of the video.  These methods only use the convolution kernel for the spatial temporal transition. The fixed quadrate receptive fields of normal CNNs could not capture the deformable instantaneous variation. For example, when it comes to fast movement, deformation and other varying motions, these predictive models may behave worse. TrajGRU \cite{shi2017deep} and non-local ConvLSTM \cite{xu2019non} take the whole feature map into account, but overlook the origin motion consistency in videos which could make the transition with more randomness. 

%Considering this property of video motions, our approach presents the MotionRNN unit which contains a learned filter with temporal information.



%from the long-term view, we find the subject motions follow a tendency with high consistency but random offsets in short-term.

%Previous predictive networks such as ConvLSTM, PredRNN only use the convolution kernel for the spatial temporal transition. The fixed quadrate receptive fields of normal CNNs restrict the video motion modeling. Thus when it comes to fast movement, deformation and other varying motions, these networks could fail. TrajGRU and other non-local networks take the whole feature map into account, but neglected the origin motion consistency in videos which could make the transition with more randomness. Considering this property of video motions, our approach presents the MoRNN unit which contains a learned filter with temporal information.

\begin{figure}[htb]
\vskip 0.15in
\centering
\includegraphics[width=0.8\columnwidth]{cvpr2021/pic/block-new-final.pdf}
\caption{MotionRNN unit, which could modeling the instantaneous variation and sustainable variation of the motion separately. The instantaneous filter learner (blue part) is to produce the instantaneous filter $\mathcal{F}_{t}^\prime$. $\mathcal{F}_{t}^\prime$ presents the instantaneous motion. The sustainable momentum learner (red part) accumulates the motion tendency by a momentum method. The sustainable momentum $\mathcal{D}_{t}^\prime$ contains the motion of the overall video.}
\label{fig:mornn_unit}
\end{figure}

%For videos, from the long-term view, we find the subject motions follow a tendency with high consistency but random offsets in short-term. Previous predictive networks such as ConvLSTM, PredRNN only use the convolution kernel for the spatial temporal transition. The fixed quadrate receptive fields of normal CNNs restrict the video motion modeling. Thus when it comes to fast movement, deformation and other varying motions, these networks could fail. TrajGRU and other non-local networks take the whole feature map into account, but neglected the origin motion consistency in videos which could make the transition with more randomness. Considering this property of video motions, our approach presents the MoRNN unit which contains a learned filter with temporal information.


%The schematic of MoRNN unit is shown in Figure \ref{fig:mornn_unit}, which consists of three parts: 
%First, the current filter learner is to produce the filter for deformation, rotation or other current motions. Different from the deformable convolutional networks \cite{dai2017deformable}, we use ConvGRU \cite{shi2017deep} to learn the filter, which can incorporate the temporal information to learn better offsets. Second, for the time consistency, the overall tendency of the motion in the video is incorporate into the unit with the process in red. Third, the black part shows the gated combination of the transitioned state and original input.

There are three inputs of MotionGRU: input feature map $\mathcal{H}_{t}^L$, the motion filter $\mathcal{F}_{t-1}^L$, the sustainable momentum $\mathcal{D}_{t-1}^{L}$. We use a Encoder-Decoder operation for memory efficiency. The inputs $\mathcal{H}_{t}^L$ and outputs $\mathcal{X}_{t}^L$ are in the feature filed $\mathbb{R}^{C\times H\times W}$. After the encoder, the feature size is convert to $\frac{C}{4}\times \frac{H}{2}\times \frac{W}{2}$. The $\mathcal{F}_{t-1}^L$ and $\mathcal{D}_{t-1}^{L}$ are in the offset filed $\mathbb{R}^{2k^{2}\times \frac{H}{2} \times \frac{W}{2}}$ to present the motion of $k\times k$ neighbour pixels in both vertical and horizontal direction. The equations of MotionGRU are shown as follows:
\begin{equation}\label{equ:mornn_unit}
  \begin{split}
  & \mathcal{F}_{t}^\prime = \text{Instantaneous}\Big(\mathcal{F}_{t-1}^L, \text{Enc}(\mathcal{H}_{t}^L)\Big)\\
  & \mathcal{D}_{t}^L = \text{Sustainable}\Big(\mathcal{F}_{t-1}^L, \mathcal{D}_{t-1}^L\Big)\\
  & \mathcal{F}_{t}^L = \mathcal{F}_{t}^\prime + \mathcal{D}_{t}^L \\
%   & {\mathcal{X}_{t}^\prime_{:,m,n}} = \sum_{i=1}^{k^2} {\mathcal{H}_{t}^\prime}_{:,m_i^\prime,n_i^\prime}G\left(({\mathcal{F}_{t}^L}_{i,m,n},{\mathcal{F}_{t}^L}_{k^2+i,m,n})\right)  \\
%   & \mathcal{X}_{t}^\prime = \text{Motion}(\text{Enc}(\mathcal{H}_{t}^L), \mathcal{F}_{t}^L) \\
  & m_{t} = \text{Broadcast}\Big(\sigma(W_{hm}\ast \text{Enc}(\mathcal{H}_{t}^L))\Big) \\
  & \mathcal{H}_t^\prime = m_t \odot \text{Warp}\Big(\text{Enc}(\mathcal{H}_{t}^L), \mathcal{F}_{t}^L\Big)\\
%   & \mathcal{H}_t^\prime = \bigg(\mathcal{H}_{c,m,n,i}^\prime\bigg)_{C\times H\times W\times k^2} = m_t \odot \\
%   & \left(\text{I}(\text{Enc}(\mathcal{H}_{t}^L)_{c,(m+p_{ix}+\mathcal{F}_{i,m,n}),(n+p_{iy}+\mathcal{F}_{i+k^2,m,n})})\right)_{C\times H\times W\times k^2} \\
%   &\bigg({\text{Warp}_{\text{I}}}\Big(\text{Enc}(\mathcal{H}_{t}^L),p_{ix}+\mathcal{F}_{i,m,n},p_{iy}+\mathcal{F}_{i+k^2,m,n}\Big)\bigg)_{C\times H\times W\times k^2} \\
  & g_{t} = \sigma \Big(W_{1\times 1}\ast \text{Concat}([\text{Dec}(\mathcal{H}_t^\prime ), \mathcal{H}_{t}^{L}])\Big) \\
  & \mathcal{X}_{t}^L = g_{t}\odot \mathcal{H}_{t-1}^L + (1-g_{t})\odot \text{Dec}(\mathcal{H}_t^\prime),\\
  \end{split}
\end{equation}
where $\sigma$ is the sigmoid function, $\ast$ and $\odot$ denote the convolution and the Hadamard product respectively. The \textit{Instantaneous} and \textit{Sustainable} present the instantaneous filter learner and sustainable momentum learner respectively. \textit{Broadcast} is to broadcast and transpose the $k^2\times\frac{H}{2}\times\frac{W}{2}$ tensor to $\frac{C}{4}\times\frac{H}{2}\times\frac{W}{2}\times k^2$. The \textit{Warp} donates the filter-based warp operation and can be formulated as following:
\begin{equation}\label{equ:mornn_unit_warp}
  \begin{split}
  & \text{Warp}(\mathcal{H}, \mathcal{F}) = \Big(\mathcal{H}_{c,m,n,i}^\prime\Big)_{C\times H\times M\times k^2}  \\  & = \Big(\mathcal{H}_{c,(m+p_{ix}-\mathcal{F}_{i,m,n}),(n+p_{iy}-\mathcal{F}_{i+k^2,m,n})}\Big)_{C\times H\times M\times k^2}, \\
  \end{split}
\end{equation}
where $p_{ix}=[\frac{i}{k}]-[\frac{k}{2}]$, $p_{iy}=(i\ \text{mod}\ k)-[\frac{k}{2}]$. Because the $\mathcal{F}_{i,m,n}$ is in float type, the warped pixel value is calculate by bilinear interpolation in a unit square. Thus the size of $\mathcal{H}_{t}^\prime$ is $\frac{C}{4}\times\frac{H}{2}\times\frac{M}{2}\times k^2$. The decoder process contains the $1\times 1$ convolution to convert tensor to $\frac{C}{4}\times\frac{H}{2}\times\frac{M}{2}$ and uses the deconvolution to convert to $C\times H\times M$.



\paragraph{Instantaneous filter.} 
% The idea of capturing deformable transitions is initially inspired by the deformbale convolution networks \cite{dai2017deformable}. The deformable convolution network adds 2D spatial offset to the regular grid sampling locations for free form deformation, but could not capture the temporal variations from the motion. Different from the deformable convolutional networks, 

the instantaneous filter is specifically designed to produce the filter for diffusion, deformation, rotation or other instantaneous motions. It uses the ConvGRU \cite{shi2017deep} to learn the spatiotemporal filter, which can incorporate the temporal information with spatial content to learn better offsets. The equation is as follows:
\begin{equation}\label{equ:motionGRU_unit}
  \begin{split}
  & u_t = \sigma\Big(W_{u}\ast \text{Concat}([\text{Enc}(\mathcal{H}_t^L), \mathcal{F}_{t-1}^L])\Big) \\
  & r_t = \sigma\Big(W_{r}\ast \text{Concat}([\text{Enc}(\mathcal{H}_t^L), \mathcal{F}_{t-1}^L])\Big) \\
  &z_t = \tanh\Big(W_{z}\ast \text{Concat}([\text{Enc}(\mathcal{H}_t^L), r_t \odot \mathcal{F}_{t-1}^L])\Big) \\
  & \mathcal{F}_t^\prime =  u_t \odot z_t 
   + (1-u_t) \odot \mathcal{F}_{t-1}^L. \\
  \end{split}
\end{equation}
% In fact, we have tried to add MotionGRU to the memory states of normal stacked-predictive framework, but due to the high computation cost we have to down sample the memory states which caused details lost and performance worse. On the contrary, we add the MotionGRU to the hidden state of layers to enhance the spatiotemporal transitions. For computation efficiency, we down sample the feature map to $\frac{1}{4}$ channels and $\frac{1}{4}$ feature size by convolutions with stride 2. Conducting the motion transition on the high-level space and then up sample back. To maintain the details of unchanged content, we using the output gate to control the transitioned motions and original hidden states. decoder changed to have an addition 1*1 conv.

%The instantaneous filter learner is to produce the filter for deformation, rotation or other instantaneous motions. Different from the deformable convolutional networks \cite{dai2017deformable}, we use ConvGRU \cite{shi2017deep} to learn the filter, which are specified as follows:
%which can incorporate the temporal information to learn better offsets. 

Current spatio-temporal information is encoded to $z_t$ after the reset gate $r_t$. The output is controlled by the update gate $u_t$. All these gates and hidden states are in the offset filed. Note that the output filter is the instantaneous but also based on the previous motion filters.


% where $\sigma$ is the sigmoid function, $\ast$ and $\odot$ denote the convolution operator and the Hadamard product respectively. $t$ donates the time step and $L$ donates the $L^{\textrm{th}}$ unit from the vertical view of a stacked framework.


% For memory efficiency, we employ the $1\times 1$ convolutional filter for $W_{o}$, $W_{u}$ and $W_{r}$. As shown in Figure \ref{fig:offset_unit}, the instantaneous filter learner contains a instantaneous filter $\mathcal{F}_{t}^\prime$, a transition filter $\mathcal{F}_{t}^L$, inputs $\mathcal{H}_{t}^L$ and outputs $\mathcal{X}_{t}^L$, 

%where $t$ donates the time step and the superscript and $L$ donates the $L^{\text{th}}$ unit from the vertical view of a stacked framework. 

% For more details, $t$ donates the time step and $L$ donates the $L^{\textrm{th}}$ unit from the vertical view of a stacked framework. The inputs, outputs and output gate $g_{t}$  are in $\mathbb{R}^{C\times H\times W}$ with $C$ channels and $H\times W$ feature map size. The filters $\mathcal{D}_{t}^L$, $\mathcal{F}_{t}^L$, $\mathcal{F}_{t}^\prime$ and update gate $u_{t}$, reset gate $r_{t}$ are in $\mathbb{R}^{(2\times k^2)\times H\times W}$, where $k$ donates the filter size. 
% The current filter $\mathcal{F}_{t}^\prime$ is from previous filter $\mathcal{F}_{t-1}^L$ and input $\mathcal{H}_{t}^L$. 
%The current filter learner which is in blue can be presented as follows:

% The transition filter $\mathcal{F}_{t}^L = \mathcal{F}_{t-1}^L + \mathcal{D}_{t}^L$ combines the stable part motion tendency and instantaneous transformation which could in high variance as shown in Figure \ref{fig:offset_unit}.


\paragraph{Sustainable momentum. } In the real world, motion always follows a tendency or pattern, such as car driving, echos moving and human walking, which is essential for video prediction. To get the overall motion tendency we have to get the whole frame sequence, but future frames are unreachable in prediction task. This dilemma is similar to reward prediction in reinforcement learning. To get the value function states, \textit{Temporal Difference} performs updates based on current estimates instead of the from the whole sequence. Enlightened by this, we use the $\mathcal{F}_{t-1}^L$ as the TD target in update equations and get the momentum update function as follows:
\begin{equation}\label{equ:dynamic}
  \begin{split}
  & \mathcal{D}_{t}^L = \mathcal{D}_{t-1}^L + \alpha (\mathcal{F}_{t-1}^L - \mathcal{D}_{t-1}^L), \\
  \end{split}
\end{equation}
where the $\alpha$ is the step size, which is the same as \textit{temporal difference learning}. With momentum update, the dynamic convergences to the weighted expectation of motion filter $\mathcal{F}_{t}^L$, which can be viewed as the \textbf{overall tendency} of the motions in a past period. This tendency estimation is with more coefficient along the video time. Also, by the accumulation process it can reduce the variance of the learned filter significantly, and performs as stabilizer for feature transition. 

\begin{figure}[htb]
\vskip 0.15in
\centering
\includegraphics[width=\columnwidth]{cvpr2021/pic/unit.pdf}
\caption{Feature map transition by MotionGRU. The motion filter, which is combined by instantaneous filter (blue square) and sustainable momentum (red square), reflects the coherence of the motion of filter size neighbourhood at the last state.}
\label{fig:offset_show}
\end{figure}

% The output $\mathcal{X}_{t}^L$ is controlled by the output gate $g_t$, the formulation is as follows:
% \begin{equation}\label{equ:output}
%   \begin{split}
%   & g_{t} = \sigma (W_{1\times 1}[\text{Dec}([\mathcal{F}_{t}^L \ast \text{Enc}(\mathcal{H}_{t}^{L})]), \mathcal{H}_{t}^{L}]) \\
%   & \mathcal{X}_{t}^L = g_{t}\odot \mathcal{H}_{t-1}^L + (1-g_{t})\odot \text{Dec}([\mathcal{F}_{t}^L \ast \text{Enc}(\mathcal{H}_{t}^{L})])\\
%   \end{split}
% \end{equation}
% where $\ast$ is the convolution operator and $\mathcal{F}_{t}^L \ast \text{Enc}(\mathcal{H}_{t}^{L})$ means the convolution filter is $\mathcal{F}_{t}^L$.

As shown in Figure \ref{fig:offset_show}, the MotionRNN learns the motion filter with instantaneous filter and sustainable momentum, which could capture both the instantaneous transformation and video tendency. This unit performers great in varying motion modeling by learning instantaneous and sustainable variation explicitly in the filter level.


\subsection{MotionRNN Framework}
\begin{figure}[htb]
\vskip 0.15in
\centering
\includegraphics[width=\columnwidth]{cvpr2021/pic/pipeline-final-new.pdf}
\caption{Predictive Framework with 3 layers: RNN-based networks (left), MotionRNN framework (center) which embeds MotionGRU into networks and a close look of connections of MotionGRU between layers. Our approach incorporates the MotionGRU (blue circles) into regular predictive models without change the spatiotemporal flow. MotionGRU is used as an operator to the vertical spatiotemporal flow. The blue dashed lines between stacked layers presents the Motion Content Highway.}
\label{fig:pipeline}
\end{figure}

As shown in Figure \ref{fig:pipeline}, normal RNN-based predictive frameworks is in the form of blocks that stacked vertically. MotionRNN incorporates the MotionGRU unit into the stacked layers without change the original spatiotemporal flows. With high flexibility, MotionRNN could replace the predictive frameworks as ConvLSTM, PredRNN, MIM, E3D-LSTM or others.

Because MotionGRU is designed as a encoder-decoder structure for memory efficiency, the incorporation causes the information bottleneck. We upgrade the predictive framework by adding the \textit{Motion Content Highway} between stacked blocks, which provides the content details. Besides, this highway could refines the motion and avoid the motion vanishing. To balance the motion and content information, we use the output gate to control the spatiotemporal flow. Here we reuse the output gate $o_t$ in RNNs. Take the ConvLSTM as an example, the original inputs are $\mathcal{X}_{t}^{L-1}$ from frames or last block, hidden state $\mathcal{H}_{t-1}^L$ from previous time step, memory state $\mathcal{C}_{t-1}^{L}$ from previous time step, where the subscript $t$ denotes the time step and the superscript $L\in\{1,2, \odot, K\}$ denotes the $L$th hidden layer in a stacked predictive framework. In MotionRNN, the input $\mathcal{X}_{t}^{L}$ is from the frames or last MotionGRU block and adds the additional \textit{Motion Content} $\mathcal{H}_{t}^{L-1}$. Especially, $\mathcal{X}_{t}^0$ is the input frame $\mathcal{X}_{t}$ or the predicted frame $\hat{\mathcal{X}_{t}}$. $\mathcal{H}_{t}^0$ is converted from $\mathcal{X}_{t}^0$ by the $1\times1$ convolution to have the same channels as hidden states. Thus the output of the original block is as follows:
\begin{equation}\label{equ:block_new}
  \begin{split}
    & \mathcal{H}_t^L = o_t \odot \tanh(W_{1\times1} \ast \mathcal{C}_t^L) + (1-o_t) \odot \mathcal{H}_t^{L-1}.\\
  \end{split}
\end{equation}

% In LSTM-based predictive networks, at the time step $t$, the input is the $t^{\text{th}}$ frame of the video. Following the vertical spatial temporal flow, the network outputs the prediction of $(t+1)^{\text{th}}$ frame. Based on this vision, each LSTM-based block can be viewed as a transition operation. However, the limitation of normal convolution filter makes the spatial temporal transition difficult. Our predictive framework uses the MoRNN unit as the operator to block output, with this explicit receptive filed, we can enhance the state transition for better results.

% Figure \ref{fig:pipeline} shows the predictive framework, which contains the normal LSTM-based blocks, such as ConvLSTM, PredRNN, MIM and E3D-LSTM, MoRNN units between stacked layers and skip connections. 

% \begin{equation}\label{equ:stlstm}
%   \begin{split}
%   & g_t = \tanh(W_{xg} \ast \mathcal{X}_t^{L-1} + W_{hg} \ast \mathcal{H}_{t-1}^L + b_g) \\
%   & i_t = \sigma(W_{xi} \ast \mathcal{X}_t^{L-1} + W_{hi} \ast \mathcal{H}_{t-1}^L + b_i) \\
%   & f_t = \sigma(W_{xf} \ast \mathcal{X}_t^{L-1} + W_{hf} \ast \mathcal{H}_{t-1}^L + b_f) \\
%   & \mathcal{C}_t^L = f_t \odot \mathcal{C}_{t-1}^L + i_t \odot g_t \\
%   & g_t^\prime = \tanh(W_{xg}^\prime \ast \mathcal{X}_t^{L-1} + W_{mg} \ast \mathcal{M}_t^{L-1} + b_g^\prime) \\
%   & i_t^\prime = \sigma(W_{xi}^\prime \ast \mathcal{X}_t^{L-1} + W_{mi} \ast \mathcal{M}_t^{L-1} + b_i^\prime) \\
%   & f_t^\prime = \sigma(W_{xf}^\prime \ast \mathcal{X}_t^{L-1} + W_{mf} \ast \mathcal{M}_t^{L-1} + b_f^\prime) \\
%   & \mathcal{M}_t^L = f_t^\prime \odot \mathcal{M}_t^{L-1} + i_t^\prime \odot g_t^\prime \\
%   & o_t = \sigma(W_{xo} \ast \mathcal{X}_t^{L-1} + W_{ho} \ast \mathcal{H}_{t-1}^L \\
%   & + W_{co} \ast \mathcal{C}_t^L + W_{mo} \ast \mathcal{M}_t^L + b_o) \\ 
%   & \mathcal{H}_t^L = o_t \odot \tanh(W_{1\times1} \ast [\mathcal{C}_t^L, \mathcal{M}_t^L]).\\
%   \end{split}
% \end{equation}
% where $W_{\cdot\cdot}$ is the $1\times1$ convolution.
% skip connection spatial temporal stabilizer

% In our predictive framework, the hidden state of last layer $\mathcal{H}_{t}^{L-1}$ is an spatial temporal stabilizer for ST-LSTM. The equations of ST-LSTM output in our framework presents as follows:
% \begin{equation}\label{equ:stlstm}
%   \begin{split}
%     & \mathcal{H}_t^L = o_t \odot \tanh(W_{1\times1} \ast [\mathcal{C}_t^L, \mathcal{M}_t^L]) + (1-o_t) \odot \mathcal{H}_t^{L-1}.\\
%   \end{split}
% \end{equation}

The overall equations for $K$ layers predictive frameworks are as follows, for $L=1, 2,\cdots, K-1$:
\begin{equation}\label{equ:overall}
  \begin{split}
    & \mathcal{H}_{t}^{L}, \mathcal{C}_{t}^{L} = \text{Block}(\mathcal{X}_{t}^{L-1}, \mathcal{H}_{t}^{L-1}, \mathcal{C}_{t-1}^{L}) \\
    & \mathcal{X}_{t}^{L}, \mathcal{F}_{t}^{L}, \mathcal{D}_{t}^{L} = \text{MotionGRU}(\mathcal{H}_{t}^{L}, \mathcal{F}_{t-1}^{L}, \mathcal{D}_{t-1}^{L}). \\
  \end{split}
\end{equation}

From the bottom to top the predictive blocks and MotionGRUs appears alternately with the MotionGRU as an operator to the hidden states $\mathcal{H}_{t}^L$. The top layer is a predictive blocks as follows:
\begin{equation}\label{equ:overall_last}
  \begin{split}
    & \mathcal{H}_{t}^{K}, \mathcal{C}_{t}^{K} = \text{Block}(\mathcal{X}_{t}^{K-1}, \mathcal{H}_{t}^{K-1}, \mathcal{C}_{t-1}^{K}). \\
  \end{split}
\end{equation}

Note that we can replace the proposed MotionRNN framework by other networks. Thus, MotionRNN is with high flexibility and could balance the motion and content by Motion Content Highway.



% \begin{figure*}[h]
% \vskip 0.05in
% \centering
% \subfigure[Incorporate into Prediction Nets]{
% \includegraphics[width=0.8\columnwidth]{cvpr2021/pic/pipeline.pdf}
% \label{fig:stacked_convlstm}
% }
% \hspace{2cm}
% \subfigure[MoRNN Block]{
% \includegraphics[width=0.65\columnwidth]{cvpr2021/pic/block.pdf}
% \label{fig:deeplstm}
% }
% \caption{
% The diagram is a case of 3 layers network. Normal predictive deep networks can be view as stacked LSTM blocks, which is the black part in (a). The blue part in (a) shows the approach to incorporating MoRNN into these networks by using it as a flexible operator to $\mathcal{H}_{t}^L$ and adding vertical spatial temporal skip connection as a stabilizer. MoRNN (b) models the motions with \textcolor{blue}{GRU block} and \textcolor{red}{
% Momentum block} to capture the deformation and tendency respectively}
% \label{fig:model_comparison}
% \end{figure*}



